On the Transmission-Computation-Energy Tradeoff in Wireless and Fixed Networks

In this paper, a framework for the analysis of the transmission-computation-energy tradeoff in wireless and fixed networks is introduced. The analysis of this tradeoff considers both the transmission energy as well as the energy consumed at the receiver to process the received signal. While previous work considers linear decoder complexity, which is only achieved by uncoded transmission, this paper claims that the average processing (or computation) energy per symbol depends exponentially on the information rate of the source message. The introduced framework is parametrized in a way that it reflects properties of fixed and wireless networks alike. The analysis of this paper shows that exponential complexity and therefore stronger codes are preferable at low data rates while linear complexity and therefore uncoded transmission becomes preferable at high data rates. The more the computation energy is emphasized (such as in fixed networks), the less hops are optimal and the lower is the benefit of multi-hopping. On the other hand, the higher the information rate of the single-hop network, the higher the benefits of multi-hopping. Both conclusions are underlined by analytical results.

==> figures/commands.tex <==
\newrgbcolor{lightblue}{0.7 0.7 0.9}
\newrgbcolor{lightgreen}{0.7 0.9 0.7}
\newrgbcolor{lightred}{0.9 0.7 0.7}
\newrgbcolor{darkgreen}{0.2 0.6 0.2}
\newrgbcolor{brown}{0.95 0.5 0.0}%
\newcommand{\LowerTriangularMatrix}[2]{%
  \pspolygon[linewidth=#1, fillcolor=black, fillstyle=solid](0, 0)(#2, 0)(0, #2)(0, 0)%
  \pspolygon[linewidth=#1, fillcolor=white, fillstyle=none](#2, 0)(0, #2)(#2, #2)(#2, 0)}

\newcommand{\Site}{%
  \pscircle[fillstyle=solid, fillcolor=white, linecolor=black](0, 0){3mm}%
  \rput(0mm, 3mm){\psframe[fillcolor=white, fillstyle=solid, linecolor=white](-2mm, -2mm)(2mm, 2mm)\rput(0, 0){\textcolor{darkgreen}{BS}}}%
  \rput(2.6mm, -1.5mm){\psframe[fillcolor=white, fillstyle=solid, linecolor=white](-2mm, -2mm)(2mm, 2mm)\rput(0, 0){\textcolor{red}{BS}}}%
  \rput(-2.6mm, -1.5mm){\psframe[fillcolor=white, fillstyle=solid, linecolor=white](-2mm, -2mm)(2mm, 2mm)\rput(0, 0){\textcolor{blue}{BS}}}%
}

\newcommand{\Basestation}{%
  %\pspolygon[fillstyle=solid, fillcolor=white](-2, -10)(2, -10)(0, -2)(-2, -10)
  %\psline(0, -2)(0, 0)
  %\psdots(0, 0)
  %\rput{135}(3, 2.5){$\mathbf{\downarrow}$}
  %\rput{225}(-2, 2.5){$\mathbf{\downarrow}$}
  \cnodeput[fillcolor=white, fillstyle=solid](0, -6){BS1}{\Large{BS}}%
}
\newcommand{\Relaynode}{%
\rput(0, 0){\Huge{$\Ydown$}}%
%\rput{180}(0, 5){$\lightning$}
}
\newcommand{\Hexagon}[1]{%
  \pspolygon[fillcolor=#1, fillstyle=solid](10, 0)(5, 8.6603)(-5, 8.6603)(-10, 0)(-5, -8.6603)(5, -8.6603)(10, 0)
  %\pspolygon[fillstyle=crosshatch*, hatchcolor=white, fillcolor=#1, hatchwidth=0.5pt, hatchsep=0.7pt, hatchangle=0](10, 0)(5, 8.6603)(-5, 8.6603)(-10, 0)(-5, -8.6603)(5, -8.6603)(10, 0)
}
\newcommand{\SiteA}[1]{%
  \rput(0, 0){\Hexagon{lightgray}}
  \rput(15, 8.6603){\Hexagon{lightblue}}
  \rput(0, 17.321){\Hexagon{lightred}}
  \rput(5, 14){\Basestation}

  % inner tier
  \rput(0.1503, 5.8603){\Relaynode}
  \rput(5, 3.063){\Relaynode}
  \rput(9.8497, 5.8603){\Relaynode}
  \rput(9.8497, 11.4603){\Relaynode}
  \rput(5, 14.2603){\Relaynode}
  \rput(0.1503, 11.4603){\Relaynode}

  % outer tier
  \rput(-4.2376, 3.327){\Relaynode}
  \rput(5, -2.0064){\Relaynode}
  \rput(14.2376, 3.3270){\Relaynode}
  \rput(14.2376, 13.9936){\Relaynode}
  \rput(5, 19.3270){\Relaynode}
  \rput(-4.2376, 13.9936){\Relaynode}
}
\newcommand{\SiteB}[1]{%
  \rput(0, 0){\Hexagon{lightblue}}
  \rput(15, 8.6603){\Hexagon{lightred}}
  \rput(15, -8.6603){\Hexagon{lightgray}}
  \rput(10, 6){\Basestation}

  % inner tier
  \rput(5.1503, -2.1397){\Relaynode}
  \rput(10, -4.937){\Relaynode}
  \rput(14.8497, -2.1397){\Relaynode}
  \rput(14.8497, 3.4603){\Relaynode}
  \rput(10, 6.2603){\Relaynode}
  \rput(5.1503, 3.4603){\Relaynode}

  % outer tier
  \rput(0.7624, -4.673){\Relaynode}
  \rput(10, -10.0064){\Relaynode}
  \rput(19.2376, -4.673){\Relaynode}
  \rput(19.2376, 5.9936){\Relaynode}
  \rput(10, 11.3270){\Relaynode}
  \rput(0.7624, 5.9936){\Relaynode}
}
\newcommand{\SiteAFR}[0]{%
  \rput(0, 0){\Hexagon{lightgray}}
  \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](8, 0)(5, 8.6603)(-4, 6.9282)(-8, 0)(-4, -6.9282)(4, -6.9282)(8, 0)
  \rput(15, 8.6603){%
    \Hexagon{lightblue}
    \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](8, 0)(4, 6.9282)(-4, 6.9282)(-10, 0)(-4, -6.9282)(4, -6.9282)(8, 0)}
  \rput(0, 17.321){%
    \Hexagon{lightred}
    \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](8, 0)(4, 6.9282)(-4, 6.9282)(-8, 0)(-4, -6.9282)(5, -8.6603)(8, 0)}
  \rput(5, 14){\Basestation}
}
\newcommand{\SiteBFR}{%
  \rput(0, 0){%
    \Hexagon{lightblue}
    \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](10, 0)(4, 6.9282)(-4, 6.9282)(-8, 0)(-4, -6.9282)(4, -6.9282)(10, 0)}
  \rput(15, 8.6603){%
    \Hexagon{lightred}
    \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](8, 0)(4, 6.9282)(-4, 6.9282)(-8, 0)(-5, -8.6603)(4, -6.9282)(8, 0)}
  \rput(15, -8.6603){\Hexagon{lightgray}
    \pspolygon[linearc=.2,fillcolor=white, fillstyle=solid](8, 0)(4, 6.9282)(-5, 8.6603)(-8, 0)(-4, -6.9282)(4, -6.9282)(8, 0)}
  \rput(10, 6){\Basestation}
}
\newcommand{\ScaledPart}[2]{%
  \begingroup
    \psset{xunit=#1, yunit=#1}
    #2
  \endgroup
}

\endinput


==> figures/table.WINNER.system.parameters.tex <==
\begin{tabular}{|p{2.8cm}|p{5cm}|}%final editing
%\begin{tabular}{|p{5cm}|p{6.0cm}|}
  \hline
  User density & \begin{minipage}{5.0cm}\vspace{0.1cm}$90$ per $\text{km}^2$ in Wide-area,\\ $250$ per $\text{km}^2$ in Manhattan-area\vspace{0.1cm}\end{minipage} \\ \hline
  Average no. users/cell & $26$ in Wide/Manhattan-area\\ \hline
  Channel models & as defined in \cite{WINNER.D1.1.1.2006} \\ \hline
  Number of antennas BS/RN/UT & $4$ / $1$ / $1$ \\ \hline
  BS transmit power  &  $\unit[46]{dBm}$ \\ \hline
  RN transmit power &  $\unit[37]{dBm}$ \\ \hline
  UT transmit power &  $\unit[24]{dBm}$ \\ \hline
  Noise figure & $\unit[7]{dB}$ \\ \hline
  Noise power spectral density & $\unit[-174]{dBm/Hz}$ \\ \hline \hline
  FFT-Size & 2048\\ \hline
  Carrier frequency & $\unit[3.95]{GHz}$ \\ \hline
  System bandwidth & $\unit[100]{MHz}$ \\ \hline
  OFDM-Symbol duration & $\unit[20.48]{\mu s}$ \\\hline
  Superframe duration & $\unit[5.89]{ms}$ \\\hline
  Guard interval & $\unit[2.00]{\mu s}$ \\ \hline
  Used subcarriers & $[-920; 920] \setminus \left\{0\right\}$ \\ \hline
  Channel state information & \begin{minipage}{5.0cm}\vspace{0.1cm}assumed to be perfectly known at transmitter and receiver\vspace{0.1cm}\end{minipage}\\ \hline
  \multirow{3}{*}{\begin{minipage}{2.8cm}Channel models according to \cite{WINNER.D1.1.2.2007}\end{minipage}} &  
  BS to RN: B5a \\ \cline{2-2}
  ~ & BS to outdoor UT: C2 \\ \cline{2-2}
  ~ & RN to outdoor UT: C2 \\ \hline
\end{tabular}


